On Minimizing the Maximum Age-of-Information For Wireless Erasure Channels

Age-of-Information (AoI) is a recently proposed metric for quantifying the freshness of information from the UE's perspective in a communication network. Recently, Kadota et al. [1] have proposed an index-type approximately optimal scheduling policy for minimizing the average-AoI metric for a downlink transmission problem. For delay-sensitive applications, including real-time control of a cyber-physical system, or scheduling URLLC traffic in 5G, it is essential to have a more stringent uniform control on AoI across all users. In this paper, we derive an exactly optimal scheduling policy for this problem in a downlink cellular system with erasure channels. Our proof of optimality involves an explicit solution to the associated average-cost Bellman Equation, which might be of independent theoretical interest. We also establish that the resulting Age-process is positive recurrent under the optimal policy, and has an exponentially light tail, with the optimal large-deviation exponent. Finally, motivated by typical applications in small-cell residential networks, we consider the problem of minimizing the peak-AoI with throughput constraints to specific UEs, and derive a heuristic policy for this problem. Extensive numerical simulations have been carried out to compare the efficacy of the proposed policies with other well-known scheduling policies, such as Randomized scheduling and Proportional Fair.

==> simulations1.tex <==
\section{Simulations}
In this section, we simulate five scheduling policies for the binary erasure channel: 1) Max Age Policy(MA) 2) Randomized Policy(RP) 3) Max Weight Policy(MW) 4) Proportional Fair(PF) 5) Max Age Policy with Throughput Constraints(MATP). The first policy is based on Section III of this paper. The second policy chooses a random User in each time slot. The third policy was proposed in \cite{AoI_infocom}. This policy in each time slot chooses the node which maximizes $p_ih_i^2$. The fourth policy was proposed in [4]. This policy chooses the UE which maximizes $p_i/R_i(t)$ where $R_i$ is updated in every time slot as: $R_i(t + 1) = R_i(t) + \epsilon y(t)$ where y is the decision variable about the successful transmission of the packet to the destination. The fifth policy is based on Section IV of the paper. \newline 
We simulate a network with N nodes over a binary erasure channel, each of which has a probability of successful transmission $p_i$ taken from a uniform distribution. Each simulation is run for $10^5$ slots and an average over 100 simulations is taken. For the PF algorithm, the value of $\epsilon$ is chosen to be 0.1. \newline
The first two plots have been simulated for networks of size N = {2, 5, 10, 20}. These two plots have been used to compare the five policies based on two performance metrics: Average Throughput and Average Max AoI. The Average throughput has been compared with the optimal lower bound given in [2,lemma 5]. The next two plots have been simulated for the MATP policy with 20 nodes. Fig. 4 shows the average throughput change with variation in $\beta = {0.01, 0.1, 1, ... , 10^6}$. Fig. 5 shows throughput achieved for the eMBB user as $\beta$ changes. In this case probability of successful transmission for the eMBB user is taken as $p_1 = 0.8$. This provides an upper bound for the throughput achievable by the policy. \newline

 


==> simulations2.tex <==
\section{Simulations} \label{simulation}
In this section, we simulate five scheduling policies for the binary erasure channel: 1) Max Age Policy(MA) 2) Randomized Policy(RP) 3) Max Weight Policy(MW) 4) Proportional Fair(PF) 5) Max Age Policy with Throughput Constraints(MATP). The first policy is based on Section III of this paper. The second policy chooses a random User in each time slot. The third policy was proposed in \cite{AoI_infocom}. This policy in each time slot chooses the node which maximizes $p_ih_i^2$. The fourth policy was proposed in [4]. This policy chooses the UE which maximizes $p_i/R_i(t)$ where $R_i$ is updated in every time slot as: $R_i(t + 1) = R_i(t) + \epsilon y(t)$ where y is the decision variable about the successful transmission of the packet to the destination. The fifth policy is based on Section IV of the paper. \newline 
We simulate a network with N nodes over a binary erasure channel, each of which has a probability of successful transmission $p_i$ taken from a uniform distribution. Each simulation is run for $10^5$ slots and an average over 100 simulations is taken. For the PF algorithm, the value of $\epsilon$ is chosen to be 0.1. \newline
The first two plots have been simulated for networks of size N = {2, 5, 10, 20}. These two plots have been used to compare the five policies based on two performance metrics: Average Throughput and Average Max AoI. The Average throughput has been compared with the optimal lower bound given in [2,lemma 5]. The next two plots have been simulated for the MATP policy with 20 nodes. Fig. 4 shows the average throughput change with variation in $\beta = {0.01, 0.1, 1, ... , 10^6}$. Fig. 5 shows throughput achieved for the eMBB user as $\beta$ changes. In this case probability of successful transmission for the eMBB user is taken as $p_1 = 0.8$. This provides an upper bound for the throughput achievable by the policy. \newline 



\begin{figure}
%\vspace{-60pt}
%\hspace{-40pt}
\centering
\begin{overpic}[width=0.4\textwidth]{./Simulation_Codes/plots/New_Plots/Avg_AoI_1}
\end{overpic}
%\vspace{-40pt}
\put(-150,142){\footnotesize{MA}}
\put(-150,131){\footnotesize{MW}}
\put(-150,121){\footnotesize{Randomized}}
\put(-150,110){\footnotesize{PF}}
\put(-150,100){\footnotesize{Optimal AoI}}
\put(-150,90){\footnotesize{(Theoretical)}}
\put(-132,0){\footnotesize{Number of UEs}}
\put(-210,50){\rotatebox{90}{\footnotesize{Long Term Max-Age}}}
\caption{\small {Comparative Performance of the Proposed Max-Age (MA) policy with three other Scheduling Policies with varying the number of UEs.}}
\label{fig:model}
\end{figure}

\begin{figure}
%\vspace{-60pt}
%\hspace{-40pt}
\centering
\begin{overpic}[width=0.4\textwidth]{./Simulation_Codes/plots/New_Plots/beta_variation2}
\end{overpic}
%\vspace{-40pt}
%\put(-150,142){\footnotesize{MA}}
%\put(-150,131){\footnotesize{MW}}
%\put(-150,121){\footnotesize{Randomized}}
%\put(-150,110){\footnotesize{PF}}
\put(-167,125){\footnotesize{Upper-Bound of UE\textsubscript{1}}}
\put(-158, 112){\footnotesize{Throughput ($p_1$)}}
\put(-90,50){\footnotesize{Throughput of UE\textsubscript{1}}}
\put(-100,0){\footnotesize{$\beta$}}
\put(-205,24){\rotatebox{90}{\footnotesize{Throughput for the Type-II UE}}}
\caption{\small {Variation of Throughput for the Type-II (eMBB) UE with the parameter $\beta$.}}
\label{fig:model}
\end{figure}

\begin{figure}
%\vspace{-60pt}
%\hspace{-40pt}
\centering
\begin{overpic}[width=0.4\textwidth]{./Simulation_Codes/plots/New_Plots/Avg_AoI_plus_beta_Tput}
\end{overpic}
%\vspace{-40pt}
%\put(-150,142){\footnotesize{MA}}
%\put(-150,131){\footnotesize{MW}}
%\put(-150,121){\footnotesize{Randomized}}
%\put(-150,110){\footnotesize{PF}}
%\put(-167,125){\footnotesize{Upper-Bound of UE\textsubscript{1}}}
%\put(-158, 112){\footnotesize{Throughput ($p_1$)}}
%\put(-90,50){\footnotesize{Throughput of UE\textsubscript{1}}}
\put(-120,0){\footnotesize{Number of UEs}}
\put(-208,15){\rotatebox{90}{\footnotesize{Long-Term Max-Age+$\beta \times$ UE\textsubscript{1} throughput}}}
\caption{\small {Comparative Performance .}}
\label{fig:model}
\end{figure}






























